Gaussian3Diff: 3D Gaussian Diffusion for 3D Full Head Synthesis and Editing

We present a novel framework for generating photorealistic 3D human head and subsequently manipulating and reposing them with remarkable flexibility. The proposed approach leverages an implicit function representation of 3D human heads, employing 3D Gaussians anchored on a parametric face model. To enhance representational capabilities and encode spatial information, we embed a lightweight tri-plane payload within each Gaussian rather than directly storing color and opacity. Additionally, we parameterize the Gaussians in a 2D UV space via a 3DMM, enabling effective utilization of the diffusion model for 3D head avatar generation. Our method facilitates the creation of diverse and realistic 3D human heads with fine-grained editing over facial features and expressions. Extensive experiments demonstrate the effectiveness of our method.

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

%-------------------------------------------------------------------------
% Background
% Generating high-quality 3D head avatars is one of the cruxes of computer vision and graphics. The generated head avatar can be used for a variety of downstream applications in the metaverse, \eg, virtual reality (VR) and augmented reality (AR).


% 3D digital avatars are the north star for human communication and self-expression in virtual or augmented reality applications.
% Users not only want their avatars to represent their identities and actions with high fidelity, but also to have full control of their perceived appearance.
% In the context of 3D head avatars, it requires us to develop
% \textbf{1)} a representation that supports accurate reenactment of the facial expressions of a real human with high visual quality.
% \textbf{2)} a method that supports user-friendly and fine-grained or even high-level editing of the avatars.

% Indeed, achieving faithful animation and user-friendly editing of the avatar have been the one of the main themes in a plethora of research in computer vision and graphics.
% With the pioneering work of 3D morphable models (3DMM)~\cite{FLAME:SiggraphAsia2017,blanz2023morphable}, model-based 3D avatar representation~\misscite[SMPL,FLAME,SMPLX,GHUM] keeps pushing the quality of geometric reconstruction and animation.
% It comes with the merits of statistically-regressed latent space and well-defined topology, but at the same time the drawback due to the difficulty in modelling complex volumetric appearances.
% On the other hand, with advancements in neural volumetric rendering~\misscite[survey], model-free approaches~\misscite[unsup3d pigan,eg3d,panohead] have made great progress in generating photo-realistic 3D portraits.
% These methods are typically based on Multi Layer Perceptron (MLP) \misscite{}, voxel grids \misscite{} or tri-planes \misscite{}, where the control and animation of the underlying geometry is not the priority by design.
% Based on these approaches, researchers have developed editing methods based on the idea of style-transfer~\cite{}, distillation~\cite{}, however still with limited controllability and quality.
% For animation, researchers have also explored hybrid representations \misscite{} with impressive visual quality, though they are often optimized for a single subject only.
% It is often not straightforward to perform editing and it often requires additional per-subject optimization.

Generating 3D-aware photorealistic portraits is one of the cruxes of computer vision and graphics, with a variety of computer graphics applications, from virtual reality (VR), augmented reality (AR) to immersive gaming and beyond. In this context, there has been a growing interest in synthesizing high-fidelity 3D portraits.
Specifically, 3D-aware GANs~\cite{Chan2021piGANPI, Chan2021EG3D, Schwarz2020NEURIPS} have been proposed to support 3D portrait generation. Early on, global NeRF-based generators~\cite{Chan2021piGANPI,pan2021shadegan} were developed to generate view-consistent portraits using volumetric representations. However, these representations are memory-inefficient and can only synthesize images with limited resolution and fidelity.
To address this issue, several approaches~\cite{Chan2021EG3D, gu2021stylenerf, tan2022volux} proposed to introduce a CNN-based upsampler for high-resolution generation. Recently, Panohead~\cite{An_2023_CVPR} is a 3D GAN that can synthesize high-quality full 3D head models in $360\degree$. Despite these advancements, none of these models possess the ability to generate editable 3D portraits.

On the other hand, FENeRF~\cite{sun2021fenerf} and IDE-3D~\cite{sun2022ide} were introduced for the purpose of portrait generation and editing. Notably, IDE-3D~\cite{sun2022ide}  facilitates local face editing through the introduction of a global triplane-based NeRF generator, leveraging semantic segmentation for conditional generation. However, since global triplanes are used to represent portraits, it is challenging to edit local facial features (e.g., nose shape) without affecting the overall appearance. Additionally, since segmentation maps are used to edit the expression, the generated portrait cannot be animated by cross-identity. Furthermore, IDE-3D is limited to synthesis human heads in near-frontal views.

We hereby present \nickname{}, a generative framework for 3D head avatar generation that enables high-level and fine-grained control over facial shape and texture, as well as expression editing. Our framework consists of two main contributions.
%
First, we introduce a novel representation of the 3D head, in which complex volumetric appearances are divided into small 3D blobs and anchored to a 3DMM face model. This allows us to decouple the low-frequency geometric deformation from the complex change in volumetric appearance, making it easy to animate using the underlying 3DMM. Technically, each blob can be represented in a pixel in the texture map of the 3DMM, and at each pixel we stored a 3D Gaussian that defines its influence region, and a small tri-plane that models the local volumetric appearance. We can therefore compute the radiance field by simply blending the results from each blob efficiently.
%
Second, in order to perform fine-grained or high-level editing using our representation, all 3D heads must be statistically related to each other. To this end, we propose a novel analysis-by-synthesis approach in which we simultaneously reconstruct large amounts of 3D heads and learn a shared latent space via auto-decoder with multi-view supervision. Given a well-defined space of 3D heads, we can then take advantage of diffusion models to achieve diverse generation and user-friendly and fine-grained editing.


We demonstrate the effectiveness of our framework by following a DatasetGAN~\cite{zhang21datasetgan} paradigm, where the experiments are conducted on samples generated from a 3D-aware GAN, \ie, Panohead~\cite{An_2023_CVPR}, which ensures us good enough fidelity and diversity.
Trained on piles of {\it single-expression} identities only, \nickname{} achieves high-quality 3D reconstruction with the intrinsic support for 3DMM-drivable animation, and compares favourably to existing volumetric avatar generation approaches, as will be shown in Sec.\label{}.
Furthermore, we use a diffusion model trained on our reconstructed avatars to showcase the superior editing ability of our framework. In Sec.\label{} we demonstrate the results for inter-subject attribute transfer, and various fine-grained editing tasks such as local region based editing, 3D in-painting with appealing visual quality.

% Existing works, model-based 
% \suggestion{This paragraph starts out being about the goal and applications, but here it switches to related work for the rest of the paragraph. It might be good to finish up a description of the goal first. What is the goal of this project? Then a paragraph explaining what exists today and their limitations makes sense afterwards.}
% \di{Maybe we can emphasize that we treat both avatar editing and animation in the same generative model framework, and in that context it's crucial to choose the right 3D representation.}

% With expressive implicit neural representations~\misscite[mlp,voxel,tri-plane], the synthesized avatars can break the constraints of mesh~\misscite[] and achieve higher fidelity.
% neural render - photorealitic, but global representation lacks animatability, topology requried for detailed editing.

% With the pioneering work of 3DMM~\cite{FLAME:SiggraphAsia2017,blanz2023morphable}, model-based 3D avatar representation~\misscite[SMPL,FLAME,SMPLX,GHUM] keeps pushing the boundary with the merits of statistically-regressed latent space, well-defined topology, and drivable property.
% % 
% With recent advancements in neural rendering~\misscite[survey], model-free~\misscite[unsup3d pigan,eg3d,panohead] have made great progress in generating photo-realistic 3D portraits.
% With expressive implicit neural representations~\misscite[mlp,voxel,tri-plane], the synthesized avatars can break the constraints of mesh~\misscite[] and achieve higher fidelity.
% neural render - photorealitic, but global representation lacks animatability, topology requried for detailed editing.

% Motivation, know issues, gap
% and model-free (global inr)

% model-based, animatable, strict topology - not flexible and photorealistic.
% \yslan{include more about the differences with previous work, limitations.}
% Though bearing high quality and flexibility, there are two underestimated limitations of the current 3D portrait generation method:
% \di{below are the desirable features, not limitations. Description can also be more concise}
% 
% \textbf{1.)} The method should support user-friendly and fine-grained editing. The user should be able to easily and precisely modify the 3D head model, such as changing the appearance and shape of facial features, \eg, skin color. 
% 
% This is important for avatar personalization in VR/AR, where the user needs to interact with the 3D head naturally and intuitively. 
% With a global representation like tri-plane~\misscite[], existing methods~\misscite[] fail to edit a specific region without affecting the other regions.
% 
% \textbf{2.)} The generated 3D human heads should be drivable by an underlying basic model. 
% This is indispensable for applying generated 3D heads to real-world applications, \ie, the 3D head model should support reenactment and accurately reproduce the facial expressions of a real human.
% Albeit previous methods made attempts to link the 3DMM latent space with the generative model latent space~\misscite[ayush,iccv,siga], 
% \yslan{fine-grained control} \di{or you want to say reenactment?} is still bounded by the learned model capacity.

% our method, Gaussian-blended local inr can combine the best of both.
% In this paper, we propose a versatile framework for 3D portrait generation, \nickname{}, to address the aforementioned problems.
% 
% The core of our method is a new implicit representation~\misscite[] composed of local 3D Gaussians to represent 3D human heads \yslan{in the UV space, suggested by YD}.
% Gaussian, 3dmm init, triplane, uv (consistent semantics)
% Specifically, a tiny 3D Gaussian~\misscite[nerflets,splatting,metaball] handles the color and geometry within its own region, and by blending Gaussians nearby, we can query the properties of a specific 3D point and render the whole scene with volume rendering~\misscite[].
% \di{It's not clear that Gaussian blending is a pre-requisite for volume rendering. Unlike simple Gaussian splatting that can only handle piece-wise constant appearance, I can imagine local tri-planes alone also allows some volumetric rendering. So I am wondering how we can justify the blending, e.g. like it allows smoother transitioning?}
% To get the best of model-based representations, a basic face model (3DMM) is adopted to initialize the underlying geometry of a 3D human head, where the center and rotation of the Gaussians are determined by the mesh vertices.
% % 
% \di{I would suggest introduce Gaussian and local tri-planes together}
% To improve the representation capacity, 
% we further augment each Gaussian with a local tri-plane. 
% These tri-plane features encode spatial information about the shape and texture within its region. 
% % 
% \yslan{needs to lint according to the above paragraph.}
% To support content generation, \nickname{} can be rasterized into the compact UV space to learn a diffusion prior~\misscite[adm].
% This representation allows us to naturally support animation and fine-grained local editing without sacrificing high fidelity.
% \suggestion{It can help an intro to briefly discuss the experiments, results, and conclusions too-- explaining why the experiments are relevant to the conclusions you want to make and the method you propose helps tie the story together.}
% \yslan{
% To balance fidelity and diversity, we follow a Sim2Real~\misscite paradigm to conduct experiments on samples from 3D-aware GAN, \ie, Panohead~\cite{An_2023_CVPR}.
% % 
% Trained on piles of single-expression identities, \nickname{} achieves high-quality 3D reconstruction with intrinsic support of 3DMM-drive animation and geometry-texture transfer ability. Moreover, our UV-space representation facilitates diffusion model training and enables local editing and 3D in-painting.
% }

% summary
% In summary, we propose a novel avatar representation, \nickname{}, 
% that facilitates high quality 3D human head avatar generation, animation and editing. 
% 
% Our method holds the merits of both model-based representations' animatability, and the flexibility and capacity of model-free representations. 
% 
% Experiments show that \nickname{} outperforms previous methods qualitatively and quantitatively.


==> sec/3_preliminary.tex <==
\section{Preliminary}
\label{sec:preliminary}
\heading{3D Gaussians}
\label{sec:3d_gaussian_preliminary}
%
\di{I would suggest make this more concise. We can describe the volume rendering here. This includes how to obtain the radiance from a tri-plane in the local coordinate space, transformation from world coordinate to local coordinate for each Gaussian, and the KNN selection with blending.
Then we can talk about the overall generative model framework that encompasses editing and animation.
Finally, we can spend more efforts on the technical details for fitting and training diffusion models}
On par with MLP-based representation~\cite{mildenhall2020nerf}, researchers also proposed 3D Gaussians~\cite{genova2019learning, genova2020local, kerbl20233d} to represent 3D scenes. Gaussians can effectively approximate coarse structures, enabling fast rendering and offering desirable editing capabilities.
% 
Specifically, each 3D Gaussian has 9 degrees of freedom:  a 3D center $\bfmu_i$, 3 axis-aligned radii, and 3 rotation angles. 
%
These parameters are utilized in rasterizing 3D Gaussians by transforming an ellipsoid into the image space.

In addition to their use in rasterization~\cite{zhang2023nerflets,kerbl20233d}, these 9 parameters also define an influence function $g_i(\bfx)$, which is an analytic radial basis function (RBF) based on scaled anisotropic multivariate Gaussians~\cite{genova2019learning, genova2020local}
% 
\begin{align}
\label{eq:influence_fun}
g_i(\bfx)=\eta\exp \left(-\frac{1}{2\tau}\left(\bfx-\bfmu_i\right)^T \Sigma_i^{-1}\left(\bfx-\bfmu_i\right)\right).
\end{align}
% 
Above, $\bfmu_i$ is the center of the basis function and $\Sigma_i$ is a 6-DOF covariance matrix determined by 3 Euler-angle rotation angles and 3 axis-aligned radii. 
% 
$\eta$ is a scaling hyper-parameter set to 5 for all experiments, and $\tau$ is a scheduled temperature hyper-parameter used to control the falloff hardness. 
% 
3D Gaussian provides a fast and compact way to evaluate a region of influence without evaluating any neural network, which is crucial for our fast training and evaluation.



% \heading{Tri-plane Hybrid 3D Representation}
% \yslan{switch to Tri-Plane and factorized representation:}
% Tri-plane~\misscite{eg3d,occnet} lies in a type of factorized 3D representation~\misscite{} with three axis-aligned orthogonal feature planes, each with resolution $S_x \times S_y \times C$ where $S_x, S_y$ denote the spatial resolution and $C$ the channels.
% % 
% Given a 3D point $\point \in \real^3$, the corresponding feature vector $(F_{xy},F_{xz},F_{yz})$ are retrieved via axis-aligned projection and bilinear interpolation.
% % 
% The summed features are decoded into $\{\bm{c},\sigma\} = p_{\psi}(\point)$ with NeRF decoder $p_{\psi}(\circ)$, where $\bm{c}$ is the radiance (color) and $\sigma$ is the volume density.

==> sec/figures/ablation-AD.tex <==
\begin{figure}[ht]
  \includegraphics[width=0.5\textwidth]{sec/figures/figures_folder/abla-ad.pdf} 
%   \includegraphics[]{example-image} 
  \caption{\textbf{Ablation Study on autodecoder.} We first reconstruct two instances individually without a shared convolutional decoder and show the texture transfer in row$-1$, and animation results in row$-2$. Visually inspected, the baseline design lacks the ability to learn unseen missing features from other instances, \eg, teeth and diverse expression. Our design shows better generality and scalability.}
\label{fig:abla:autodecoder}
\end{figure}

==> sec/figures/ablation-knn.tex <==
\begin{figure}[h!]
  \includegraphics[width=0.5\textwidth]{sec/figures/figures_folder/abla-knn.pdf}
%   \caption{\textbf{Qualitative Ablation of $K$ in gaussian Blending.} 
%   Though achieving comparative quantitative performance, smaller $K$ yields visually more noisy reconstruction, as we highlight in the \textcolor{red}{red box}. Setting $K=5$ improves smoothness, as shown in 
%   the \textcolor{green}{green box}. We adopt $K=3$ to balance the overall performance.
%   All results are obtained from auto-decoder $\decoder$ directly without super resolution.
%   }
\caption{\textbf{Qualitative Ablation of $K$ in Gaussian Blending.} Despite achieving comparable quantitative performance, a smaller $K$ results in visually noisier reconstruction, as shown in the \textcolor{red}{red box}. Setting $K=5$ enhances smoothness, as illustrated in the \textcolor{green}{green box}. We opt for $K=3$ to strike a balance in overall performance. All results are obtained directly from the auto-decoder $\decoder$, without employing super resolution.}
\label{fig:abla:knn}
\end{figure}

==> sec/figures/application-diffusion-geo-tex-inpaint.tex <==
% \begin{figure}[h!]
\begin{figure*}[ht]
  \includegraphics[width=1\textwidth]{sec/figures/figures_folder/geo-tex-inpainting.pdf}
  \caption{\textbf{Diffusion-based Inpainting given Geometry or Texture Mask.} 
%   We provide with the geometry-part (first $9$ channels of the $256\times256\times33$ of $\gaussian_0$) 
%   or the texture-part (last $24$ channels of the $256\times256\times33$ of $\gaussian_0$) of the upper face as the hints, and let the diffusion model $f_\theta$ in-paints the remaining. As shown in column $2-5$, all the generated results have identical upper-face shape, \eg, eyes and forehead layout, but with different textures; 
%   while all the texture-masked diffusion in-painted results (column $6-10$) have identical upper-face texture, \eg, hair and forehead color, but with different shape.
We provide either the geometry part (first $9$ channels of the $256\times256\times33$ tensor $\gaussian_0$) or the texture part (last $24$ channels of the $256\times256\times33$ tensor $\gaussian_0$) of the \emph{upper face} as hints, and take the diffusion model $f_\theta$ in-paints the remaining details. 
% 
As illustrated in columns $2-5$, all the generated results exhibit an identical upper-face shape, including the layout of the eyes and forehead, but with different textures. Conversely, the diffusion-inpainted results with texture masks (columns $6-10$) showcase an identical upper-face texture, encompassing features such as hair and forehead color, while varying in shape.
  }
  \vspace{-2mm}
\label{fig:application:diffusion:geo-tex-inpaint}
\end{figure*}
% \end{figure}

==> sec/figures/application-diffusion-tex-inpaint.tex <==
\begin{figure}[h!]
  \includegraphics[width=0.5\textwidth]{sec/figures/figures_folder/diffusion-texture-inpainting.pdf}
  \caption{\textbf{Diffusion-based Inpainting given Texture Mask.} 
  We provide with the texture-part (last $24$ channels of the $256\times256\times33$ of $\gaussian_0$) of the upper face as the hints, and let the diffusion model $f_\theta$ in-paints the remaining. As shown here, all the generated results have identical upper-face texture, \eg, hair and forehead color, but with different shape.
  }
  \vspace{-2mm}
\label{fig:application:diffusion:tex-inpaint}
\end{figure}

==> sec/figures/application-id-transfer.tex <==
\begin{figure*}[ht]
  \includegraphics[width=1.0\textwidth]{sec/figures/figures_folder/id_transfer.pdf} 
%   \includegraphics[]{example-image} 
  \caption{\textbf{3DMM-based Editing}. We reenact $8$ random sampled source inputs (row-$1$) onto the targets (row-$2,3,4$) by driving the target Gaussians through the adjustment of the inner 3DMM mesh using the shape and expression codes from the source.
%   
  The reenactment results preserve their original texture while adapting to the shape and expression of the source inputs.
  }
  \label{fig:applicatin:id-transfer}
\end{figure*}

==> sec/figures/application-inversion.tex <==
\begin{figure}[t]
  \includegraphics[width=0.5\textwidth,]{sec/figures/figures_folder/inversion.pdf} 
  \vspace{-6mm}
  \caption{\textbf{Single-view inversion on the pre-trained auto-decoder $\decoder$}
  We randomly sample one image from CelebA-HQ~\cite{CelebAMask-HQ} and conduct test-time optimization to find the corresponding Gaussians. while the input view can be plausibly reconstructed, 
%   the novel view and novel expression results have noticeable artifacts.
the results for novel views and expressions exhibit noticeable artifacts.
  }
\label{fig:inversion}
  \vspace{-2mm}
\end{figure}

==> sec/figures/application-region-transfer.tex <==
\begin{figure*}[ht]
  \includegraphics[width=1.0\textwidth]{sec/figures/figures_folder/region-transfer-geo.pdf} 
%   \includegraphics[]{example-image} 
%   \caption{\textbf{Regional Editing given UV Mask}. Thanks to the UV-space design, \nickname{} supports editing a specific semantics region defined on the UV map.
% %   
%  Here, we transfer the "nose" and "mouse" geometry shape from the source identities to the target and leaving the remaining areas unchanged.
% %   
%   Note that all the source and target identities here are diffusion-sampled.
%   }
\caption{\textbf{Regional Editing with UV Mask}. The UV-space design in \nickname{} enables the editing of specific semantic regions defined on the UV map.
%   
  In this example, we transfer the geometry shapes of the "nose" and "mouth" from the source identities to the target while leaving the remaining areas unchanged.
%   
  It is important to note that all the source and target identities presented here are diffusion-sampled.
  }

  \label{fig:applicatin:region-editing}
\end{figure*}

==> sec/figures/baseline-ide3d.tex <==
\begin{figure}[h!]
  \includegraphics[width=0.5\textwidth]{sec/figures/figures_folder/animation-ide3d.pdf} 
  \vspace{-6mm}
  \caption{\textbf{Comparison with IDE-3D on Reenactment.} Employing four reference images (row-$1$), we animate the identities synthesized by IDE-3D and our method to the target expression.
%   
  Given IDE-3D's segmentation-based nature, utilizing a reference identity with a different shape inevitably alters the facial layout.
%   
  Nevertheless, \nickname{} is build on a identity-and-expression disentangled modeling, facilitated by the underlying 3DMM, ensuring the preservation of the input identity through the reenactment process.
  }
\label{fig:baseline:ide3d}
\end{figure}

==> sec/figures/clip-filter.tex <==
\begin{figure}[t]
  \includegraphics[width=0.5\textwidth]{sec/figures/figures_folder/clip-filter.pdf} 
  \vspace{-4mm}
  \caption{\textbf{Visualization of positive and negative samples from Panohead.} The display includes one positive sample and four negative samples here. The positive sample process a ``human front face'' score of $2.16e-04$, while all the negative samples process scores $\ge 0.5$.}
\label{fig:clip-filter}
\end{figure}

==> sec/figures/editing-3d-inpainting.tex <==
\begin{figure}[ht]
\label{fig:3d-inpainting}
  \includegraphics[width=0.5\textwidth,height=6cm]{example-image} 
%   \includegraphics[]{example-image} 
  \caption{3D Inpainting.}
\end{figure}

==> sec/figures/editing_transfer.tex <==
\begin{figure}[h]
%   \includegraphics[width=0.5\textwidth]{sec/figures/figures_folder/shape-tex-transfer.pdf} 
  \includegraphics[width=0.5\textwidth]{sec/figures/figures_folder/shape-tex-transfer-3c.pdf} 
  \vspace{-6mm}
  \caption{\textbf{Shape Texture Transfer.} 
  Given two randomly sampled source identities, each serving as the source of texture (columns $1-2$) and shape (columns $3-4$), we transfer their corresponding information defined in the UV space to four targets.
% 
Importantly, the transferred textures semantically adhere to the target shape; for instance, the beard in column $2$ varies according to the size of the Gaussians in that region.
% 
Additionally, the texture source identity of column $1$ does not display teeth, while the transferred results do, illustrating that the autodecoder $\decoder$ learns a shared meaningful latent space.
% 
These results, as evidenced in Fig.~\ref{fig:abla:autodecoder}, cannot be achieved via per-instance fitting.
}
\label{fig:tex-transfer}
\vspace{-4mm}
\end{figure}

==> sec/figures/vis-gaussian.tex <==
% \begin{figure}[ht]
%   \includegraphics[width=0.5\textwidth]{sec/figures/figures_folder/gaussian_visualize.pdf} 
% %   \includegraphics[]{example-image} 
%   \caption{Gaussian Visualization. Placeholder.}
% \label{fig:gaussian-visualization}
% \end{figure}

==> sec/finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/table/abla-ad.tex <==
% \begin{table}[tp]
% \centering
% \small
% {
% % \caption{\textbf{Quantitative performance.}} 
% \vspace{-2mm}
% \label{tab:abla:ad}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{l@{\hspace{3mm}}ccccccc}
% \toprule
% Methods & ID  $\uparrow$ &  Depth $\downarrow$ &   PCK@2.5 $\uparrow$  & PCK@5$\uparrow$   & FPS $\uparrow$ & Batch Size  \\
% \midrule
% FENeRF & 0.61 & 2.71 & - & - & TODO & 10 \\
% Panohead & \textbf{0.80} & {2.32} & - & - & TODO  & 72 \\
% IDE-3D & 0.76 & \textbf{1.71} & 0.16 & 0.33 & TODO & 48 \\
% \midrule
% Ours    &{0.78} & 2.58 & \textbf{0.783} & \textbf{0.99} & 42 & 8.25 \\
%  \bottomrule
% \end{tabular}}}
% \vspace{2mm}
% \end{table}

==> sec/table/abla-knn.tex <==
\begin{table}[tp]
\centering
\small
{
% \caption{\textbf{Quantitative ablation of $K$ in Gaussian Blending.} Larger $K$ yields better reconstruction at an extra computational cost. BS denotes batch size.} 
\caption{\textbf{Quantitative Ablation of $K$ in Gaussian Blending.} 
We evaluate the reconstruction results at $20K$ iterations.
Increasing the value of $K$ improves the quality of reconstruction, albeit with an associated increase in computational resources. 
% 
Nevertheless, beyond $K$=3, a decline in performance is observed, indicative of potential undertraining of the model.
% 
BS denotes batch size.}
\vspace{-2mm}
\label{tab:abla:k}
\resizebox{\linewidth}{!}{
\begin{tabular}{l@{\hspace{3mm}}ccccc}
\toprule
$K$ value & PSNR  $\uparrow$ &  MAE $\downarrow$ &   VRAM(MiB)@BS=4 $\downarrow$  & Latency(s)/step $\downarrow$  \\
\midrule
$1$ & 27.72 $\pm$ 2.53 & 0.0421 $\pm$ 0.013 & 6886 & 0.4 & \\
$2$ & 27.92 $\pm$ 2.40 & 0.0412 $\pm$ 0.012 & 11508 & 0.53 & \\
$3$ & \textbf{28.39} $\pm$ 2.55 & \textbf{0.0392} $\pm$ 0.012 & 16124 & 0.67 & \\
$4$ & 28.28 $\pm$ 2.37 & 0.0400 $\pm$ 0.012 & 20774 & 0.8 & \\
$5$ &  28.25 $\pm$ 2.33 & 0.0395 $\pm$ 0.011 & 25402 & 0.87 & \\
\bottomrule
\end{tabular}}}
\vspace{0mm}
\end{table}
